Evaluation of CT Image Synthesis Methods:From Atlas-based Registration to Deep Learning

Computed tomography (CT) is a widely used imaging modality for medical diagnosis and treatment. In electroencephalography (EEG), CT imaging is necessary for co-registering with magnetic resonance imaging (MRI) and for creating more accurate head models for the brain electrical activity due to better representation of bone anatomy. Unfortunately, CT imaging exposes patients to potentially harmful sources of ionizing radiation. Image synthesis methods present a solution for avoiding extra radiation exposure. In this paper, we perform image synthesis to create a realistic, synthetic CT image from MRI of the same subject, and we present a comparison of different image synthesis techniques. Using a dataset of 30 paired MRI and CT image volumes, our results compare image synthesis using deep neural network regression, state-of-the-art adversarial deep learning, as well as atlas-based synthesis utilizing image registration. We also present a novel synthesis method that combines multi-atlas registration as a prior to deep learning algorithms, in which we perform a weighted addition of synthetic CT images, derived from atlases, to the output of a deep neural network to obtain a residual type of learning. In addition to evaluating the quality of the synthetic CT images, we also demonstrate that image synthesis methods allow for more accurate bone segmentation using the synthetic CT imaging than would otherwise be possible by segmenting the bone in the MRI directly.

==> old_stuff.tex <==

% OLD abstract
% In the field of medical research, diagnostics and treatment CT scans are widely used, but also exposes the subject to ionizing radiation.
% In recent years, research has been carried out trying to synthesize CT images derived from other modalities, including MRI with the purpose of avoiding radiation exposure and increasing workflow efficiency. 
% Especially, deep learning techniques have proven to be useful for cross-modality estimation. This paper demonstrates that preceding methods like multi-atlas registration can serve as priors to deep learning algorithms, thus decreasing training time and increasing efficiency. 
% In particular, we do a weighted addition of synthetic CT images, derived from atlases, to the output of a deep neural network to obtain a residual type of learning. A series of experiments showed that using priors yielded better estimation with fewer parameters and faster training compared to state-of-the-art methods.




% Introduction not used parts:

%A third application used a cGAN in combination with an FCN. The FCN was trained to synthesize a PET image given a CT image. The synthesized PET was then concatenated with the CT image and used to train the cGAN, thus yielding a variation of an ACM \cite{ImgSynBlend}.

%\todo{Reread:\\doi.org/10.1007/978-3-319-67564-0\_5. I Don't understand this}
%Synthesize PET data via multi-channel generative adversarial networks (CT + label) (Only 2D) HOW DO YOU EVEN GET THE LABEL? and if you know where the high uptake regions is, then why do you need PET?
% A interesting approach to cross-modality medical image synthesis, is to extend the input data with an extra channel, that provides additional information. Notably, it turned out to be feasible to add a segmentation mask for cancerous 
% \cite{SynthesisPETwSegmentation}

% ONLY IN PRE-PRINT/ARXIV:
% Translating and Segmenting Multimodal Medical Volumes with Cycle- and Shape-Consistency Generative Adversarial Network (2018): Uses CycleGAN to synthesize MR and CT and adds a segmenter network to penalize shape differences.
%To overcome the need of paired data, a Cycle Consistent Adversarial Network (CycleGAN) can be used to synthesize MR and CT images. Noteworthy, is a proposed methods where two \textit{segmentors} was added to the CycleGAN. The segmentors perform segmentation of the images from each distribution and the mis-classification is penalized by a cross entropy loss term. This minimizes the differences in classified pixels and thereby shapes of elements in the synthesized images. This method was applied to cardiac MR and CT images, and significantly improved segmentation performance, while producing realistic looking images \cite{SynthesisSegmentor}.
% Cross-modality image synthesis from unpaired data using CycleGAN: CycleGAN MR to CT synthesis with gradient consistency loss.
%Another way to minimize the differences in synthesized images and real images is to maximize the the normalized cross correlation between each of the gradients of the two images. This forces the model to learn the alignment of edges in each dimension and should in turn produce sharper images. This strategy was shown to yield significantly sharper sCTs \cite{CycleSynGC}.



% Old contributions
%None of the presented related methods take in account prior knowledge about the nature of MRI and CT images. For most applications of synthetic CT images the main area of interest is bone features such as bone location, density, thickness, quality. The soft tissue is most often less important, and it is not necessary to spend a large amount of parameters on learning to cancel out soft tissue, when a quick and relatively good method to generate preliminary synthetic CT are available.\todo{Insert figure of MR/CT differences here}


%\subsection{The Multi-Scale U-Net}
%Finally, we introduce a novel deep neural network illustrated in figure \ref{fig:msunet}\todo{Insert figure here}, based on the architecture of the U-Net. The network is designed to internally create a multi-scale image representation by applying a Gaussian smoothing kernel to the input image while down-sampling it. The smoothed and down-sampled image is passed through a series of convolutional layers and concatenated to the feature maps of the max-pooled features of the U-Net. 

%Training on smoothed and down-sampled images intends to accelerate the learning process, by learning filter based on lower frequency information in the image. This sub-problem yields a more convex loss function and therefore guides the training. The skip connections in the regular U-Net makes sure that high-frequency information is preserved while the multi-scale part of the network should cause faster convergence.


%  denoted $A_{MRI}$, $A_{CT}$, and $A_{bone}$ respectively


% old methods stuff

\subsection{Synthesizing a Preliminary CT Image}

Initially, an atlas-based registration algorithm is used to synthesize the preliminary CT image, $S_{atlas}(I_{MRI})$. Specifically, we collect a database of five paired and aligned MRI, CT and bone mask atlases. When provided with $I_{MRI}$, each of the MRI atlas is aligned to $I_{MRI}$ using affine registration. The computed affine transformations are applied to the CT atlases and the bone mask atlases. The aligned CT atlases are averaged to produce a tentative synthesized CT image\todo{John: Please elaborate/correct the paragraph about atlas-based registration synthesis}. The aligned bone masks are averaged as well and smoothed with a Gaussian distribution parameterized the standard deviation $\sigma$. The smoothed bone mask, $W_{bone}$, is then saturated with the function:
$$
W_{bone}(i) = \bigg\{\begin{array}{lr}
        1 & \;\;\text{if}\;\; I_{bone}(i) > t \\
        \frac{I_{bone}(i)}{t} & \;\;\text{if}\;\; I_{bone}(i) \leq t
        \end{array},\;\; \forall i \in \Omega_{I_{bone}}
$$
where $t$ is a threshold such that $0 \leq t \leq 1$ and $I_{bone}(i)$ is the intensity value at index $i$ from the set of indices, $\Omega_{I_{bone}}$, in $I_{bone}$.

\subsection{Learning the Difference with a Deep Neural Network}

$W_{bone}$ provides an image that roughly locates bone and the proximity of the bone. By using $W_{bone}$ as a weight on the output of a deep neural network, we force the deep neural network to pay particular attention to the synthesis of the bone and less attention to areas outside the head and inside the skull. 

A deep neural network computes the function $S_{DNN}(I_{MRI})$. The loss function, used for training, is defined as:
$$
\mathcal{L}(S(I_{MRI}),I_{CT}) = \sum_{i \in \Omega} (S(I_{MRI})(i) - I_{CT}(i))^2
$$
which can be interpreted as a $L_2$ loss function and $\Omega$ is the set of all indices in $S(I_{MRI})$, which is the same size as $I_{CT}$. Lastly, we combine the images and calculate the weights be the following linear relationship:
$$
W_1 = \alpha W_{bone} + \beta
$$
and
$$
W_2 = 1 - W_1
$$
where $\alpha$ and $\beta$ are to be chosen such that $0 \leq W_1 \leq 1$. These parameters allow tuning of how much to weigh $S_{DNN}(I_{MRI})$ and how much to weigh $S_{atlas}(I_{MRI})$ and can be altered at any stage of the training.




%Sergei's comment: Tables 1 & 2  need to be commented in the text.  Not clear  what  is expected theoretically from  Experiments 1 and  2 – or in other words - where the synthetic CT quality will be or should be better  - in the head or within bones ? the head mask versus bone mask ?   Further - why are the particular numbers  given  in these tables good  / not very good ?  If most of the readers are familiar with Pearson Cross Correlation  ( PCC)  - the mean correlation ~ 0.95 with the ground truth  is perceived to be good, but what about less common Peak  Signal-to-Noise  Ratio  (PSNR),  MeanStructural Similarity (MSSIM), Mean Average Error (MAE)  ? Are they all consistent ? 
%For instance,  it seems that PSNR = 28 db is better that PSNR = 25 db  - and therefore  U-net is better than Atlas based method  ( the higher SNR , the better) ?  Accordingly,  in terms of MAE ( mean average error ) – the number  71.6  ( Atlas) is worse  than  44.5 ( U-net) .
%Finally – Table 3 – The ground truth for  bone template image  is segmentation of the raw true  CT image – correct ?   Then you compare it with segmentation of the synthetic CTs and segmentation of MRI (the bottom line) ?   DICE metric (except Atlas)   is ~ 0.6  - how good  it is versus ideal  1 or 100? What is the impact of spatial normalization / co-registration ina-accuracies on the final accuracy ?


% =====

\begin{table}[t]
\caption{Results of MRI to CT synthesis with all methods evaluated with PSNR, MAE, MSSIM and PCC on the head masked synthetic CT.}
\centering
\makebox[\textwidth][c]{
\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{9}{|c|}{Results of head mask synthetic CT image} \\ \hline
\multirow{2}{*}{Similarity metric} & \multicolumn{2}{c|}{PSNR} & \multicolumn{2}{c|}{MAE} & \multicolumn{2}{c|}{SSIM} & \multicolumn{2}{c|}{PCC} \\ \cline{2-9} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} \\ \hline
2D Atlas & 25.974 (1.006) & 25.999 & 71.606 (14.789) & 69.951 & 0.893 (0.031) & 0.896 & 0.94 (0.017) & 0.942 \\
2D U-Net & 28.01 (2.041) & 27.99 & 44.578 (16.642) & 42.663 & 0.911 (0.032) & 0.913 & 0.951 (0.023) & 0.956 \\
Adversarial & 27.931 (1.945) & 27.924 & 44.748 (16.344) & 42.771 & 0.91 (0.032) & 0.911 & 0.951 (0.02) & 0.954 \\
3D U-Net   &   &   &   &   &   &   &   &   \\
Boneweighted & 27.381 (1.845) & 27.536 & 56.035 (16.861) & 54.005 & 0.903 (0.033) & 0.907 & 0.946 (0.02) & 0.953 \\ \hline
\end{tabular}
}
\centering \\[1mm]
\label{res:head}
\end{table}

% =====

\begin{table}[t] 
\caption{Results of MRI to CT synthesis with all methods evaluated with PSNR, MAE, MSSIM and PCC on the bone masked synthetic CT.}
\centering
\makebox[\textwidth][c]{
\begin{tabular}{|l|ll|ll|ll|ll|}
\hline
\multicolumn{9}{|c|}{Results of bone masked synthetic CT image} \\ \hline
\multirow{2}{*}{Similarity metric} & \multicolumn{2}{c|}{PSNR} & \multicolumn{2}{c|}{MAE} & \multicolumn{2}{c|}{SSIM} & \multicolumn{2}{c|}{PCC} \\ \cline{2-9} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} & \multicolumn{1}{c}{Mean (std)} & \multicolumn{1}{c|}{Median} \\ \hline
Atlas & 38.87 (1.707) & 38.886 & 16.293 (4.231) & 15.881 & 0.928 (0.015) & 0.929 & 0.901 (0.029) & 0.903 \\
2D U-Net & 41.609 (3.023) & 41.524 & 9.089 (4.803) & 8.248 & 0.966 (0.016) & 0.971 & 0.936 (0.028) & 0.94 \\
Adversarial & 41.593 (2.877) & 41.405 & 9.034 (4.504) & 8.314 & 0.966 (0.015) & 0.969 & 0.937 (0.024) & 0.939 \\
3D U-Net   &   &   &   &   &   &   &   &   \\
Boneweighted & 41.272 (2.774) & 41.187 & 10.055 (4.533) & 9.246 & 0.962 (0.016) & 0.963 & 0.932 (0.026) & 0.939 \\ \hline
\end{tabular}
}
\centering \\[1mm]
\label{res:bone}
\end{table}
% =====


\begin{figure}[t]
\begin{center}
\missingfigure[figheight=4cm,figwidth=10cm]{Shown sCTs for different methods}
\end{center} 
\caption{TODO: Some caption.}
\label{fig:images}
\end{figure}


% =====

\begin{table}[t]
\caption{Dice overlap scores of segmenting synthetic CT image from all methods with k-means clustering of binned intensity values compared to 2D U-Net MRI bone segmentation}
\begin{tabular}{|l|cc|}
\hline
\multicolumn{3}{|c|}{Results of bone segmentation of synthetic CT image} \\ \hline
\multirow{2}{*}{Similarity metric} & \multicolumn{2}{c|}{Dice} \\ \cline{2-3} & Mean (std) & Median  \\ \hline
Atlas & 0.546 (0.079)   & 0.535   \\
2D U-Net & 0.643 (0.108)   & 0.635   \\
Adversarial & 0.646 (0.103) & 0.64 \\
3D U-Net   &   &   \\
Boneweighted & 0.63 (0.11) & 0.633 \\ \hline
\begin{tabular}[c]{@{}l@{}}U-Net segmentation\\ baseline\end{tabular} & 0.627 (0.101)   & 0.625   \\ \hline
\end{tabular}
\centering \\[1mm]
\end{table}
% =====


